Exploring the impact of low-rank adaptation on the performance, efficiency, and regularization of RLHF

During the last stage of RLHF, a large language model is aligned to human intents via PPO training, a process that generally requires large-scale computational resources. In this technical report, we empirically investigate an efficient implementation of RLHF using low-rank adaptation (LoRA), which allows us to align the LLaMA 7B checkpoint on the Alpaca dataset using only two A100 GPUs instead of the eight required for full model fine-tuning. Despite tuning only 0.2% of LLaMA 7B's parameters, our implementation achieves better performance than the publicly-released AlpacaFarm checkpoint with full model fine-tuning. Next, we analyze several configurations of our LoRA-based PPO implementation, varying the form of the KL regularization term in the training objective. We find that (1) removing this penalty term does not harm performance on the AlpacaFarm evaluation set under our LoRA setup; (2) other regularizers, such as Jensen-Shannon divergence, lead to improved performance; and (3) while PPO training negatively impacts the factuality of model-generated responses, training with LoRA largely mitigates this effect. We release our code and pretrained checkpoints to facilitate future research on more efficient RLHF.

==> sections/experiments.tex <==
\section{Experiments}

% alpaca_farm dataset and base models

% some conclusions
% compare different kl
% compare same kl, but different dropout and bsz
% is kl really necessary? if drop the kl term, implications: reduce memory consumption





% \paragraph{Other Details \& Discussion} As the fully-sharded parallel~\citep{zhao2023pytorch}, till the time we conduct our experiments, does not fully support disabling gradients for selected parameters, we did not use any sort of model parallelism in our experiments. Instead, we store the policy and value on one GPU, and the reference policy and reward model on the other. This has two severe limitations: (1) the GPU that stores reward and reference policy is only sparsely utilized; (2) this setting may not generalize well to models larger than 7B parameters. Nevertheless, we adopt this setting for the time being.



